The i-process yields of rapidly-accreting white dwarfs from multicycle He-shell flash stellar evolution models with mixing parameterizations from 3D hydrodynamics simulations

We have modelled the multicycle evolution of rapidly-accreting CO white dwarfs (RAWDs) with stable H burning intermittent with strong He-shell flashes on their surfaces for $0.7\leq M_\mathrm{RAWD}/M_\odot\leq 0.75$ and [Fe/H] ranging from $0$ to $-2.6$. We have also computed the i-process nucleosynthesis yields for these models. The i process occurs when convection driven by the He-shell flash ingests protons from the accreted H-rich surface layer, which results in maximum neutron densities $N_\mathrm{n,max}\approx 10^{13}$-$10^{15}\ \mathrm{cm}^{-3}$. The H-ingestion rate and the convective boundary mixing (CBM) parameter $f_\mathrm{top}$ adopted in the one-dimensional nucleosynthesis and stellar evolution models are constrained through 3D hydrodynamic simulations. The mass ingestion rate and, for the first time, the scaling laws for the CBM parameter $f_\mathrm{top}$ have been determined from 3D hydrodynamic simulations. We confirm our previous result that the high-metallicity RAWDs have a low mass retention efficiency ($\eta < 10\%$). A new result is that RAWDs with [Fe/H]$< -2$ have $\eta > 20\%$, therefore their masses may reach the Chandrasekhar limit and they may eventually explode as SNeIa. This result and the good fits of the i-process yields from the metal-poor RAWDs to the observed chemical composition of the CEMP-r/s stars suggest that some of the present-day CEMP-r/s stars could be former distant members of triple systems, orbiting close binary systems with RAWDs that may have later exploded as SNeIa.

==> vectors.tex <==
%=======================================================================
%
% vectors.tex---some basic vector operators
%
% Requires package bm.sty
%
%=======================================================================

\RequirePackage{bm}
%\RequirePackage{amssymb}
%\RequirePackage{amsbsy}
\newcommand{\bvec}[1]{\ensuremath{\boldsymbol{#1}}} %boldface vector style
\newcommand{\grad}{\bvec{\nabla}} %gradient
\newcommand{\divr}{\nabla \cdot} %divergence
\newcommand{\curl}{\bvec{\nabla \times}} %curl
\newcommand{\lap}{\ensuremath{\nabla^2}} %Laplacian
\newcommand{\btens}[1]{\ensuremath{\boldsymbol{\mathsf{#1}}}}
\newcommand{\vcross}{\bvec{\times}}
\newcommand{\vdot}{\bvec{\cdot}}
% end vectors.tex

